Fair-SSL: Building fair ML Software with less data

Ethical bias in machine learning models has become a matter of concern in the software engineering community. Most of the prior software engineering works concentrated on finding ethical bias in models rather than fixing it. After finding bias, the next step is mitigation. Prior researchers mainly tried to use supervised approaches to achieve fairness. However, in the real world, getting data with trustworthy ground truth is challenging and also ground truth can contain human bias. Semi-supervised learning is a machine learning technique where, incrementally, labeled data is used to generate pseudo-labels for the rest of the data (and then all that data is used for model training). In this work, we apply four popular semi-supervised techniques as pseudo-labelers to create fair classification models. Our framework, Fair-SSL, takes a very small amount (10%) of labeled data as input and generates pseudo-labels for the unlabeled data. We then synthetically generate new data points to balance the training data based on class and protected attribute as proposed by Chakraborty et al. in FSE 2021. Finally, the classification model is trained on the balanced pseudo-labeled data and validated on test data. After experimenting on ten datasets and three learners, we find that Fair-SSL achieves similar performance as three state-of-the-art bias mitigation algorithms. That said, the clear advantage of Fair-SSL is that it requires only 10% of the labeled training data. To the best of our knowledge, this is the first SE work where semi-supervised techniques are used to fight against ethical bias in SE ML models.

==> options.tex <==
\begin{table}

%\captionsetup{font=footnotesize}
\caption{Hyperparameter  options
seen in recent SE papers~\cite{ghotra2015revisiting,fu2016tuning,agrawal2018better,agrawal2018wrong} and in  the documentation of a widely-used data mining library
(Scikit-learn~\cite{pedregosa2011scikit}) for a list of options not explored
in those studies.
While this list is incomplete, it does include many
of the   hyperparameter optimizations being explored in the literature. }\label{tbl:options}
\footnotesize
 
\begin{tabular}{|p{.95\linewidth}|}\hline
\textbf{Learners:}  


\noindent
\bi
\item DecisionTreeClassifier(criterion=b, splitter=c, min\_samples\_split=a)
    \bi
   \item a, b, c= randuniform(0.0,1.0), randchoice([`gini',`entropy']), \newline randchoice([`best',`random'])
   \ei
\item RandomForestClassifier(n\_estimators=a,criterion=b,  min\_samples\_split=c)
    \bi
   \item a,b,c = randint(50, 150), randchoice(['gini', 'entropy']),\newline randuniform(0.0, 1.0) 
   \ei
\item LogisticRegression(penalty=a, tol=b, C=float(c))
    \bi
    \item a,b,c=randchoice([`l1',`l2']), randuniform(0.0,0.1), randint(1,500)
    \ei 
\item MultinomialNB(alpha=a) = randuniform(0.0,0.1)
\item KNeighborsClassifier(n\_neighbors=a, weights=b, p=d, metric=c)
    \bi
    \item a, b,c  = randint(2, 25), randchoice([`uniform', `distance']), \newline randchoice([`minkowski',`chebyshev'])
    \item if c=='minkowski': d= randint(1,15)  else:  d=2
    \ei
     
    
\ei
\\\hline

{\bf Pre-processors for   defect prediction, Issue lifetime, Bad   Smells:} 

\bi 
\item StandardScaler
\item MinMaxScaler
\item MaxAbsScaler
\item RobustScaler(quantile\_range=(a, b)) =  randint(0,50), randint(51,100) 
\item KernelCenterer
\item QuantileTransformer(n\_quantiles=a,  output\_distribution=c, subsample=b)
    \bi
    \item a, b = randint(100, 1000), randint(1000, 1e5)
    \item c = randchoice([`normal',`uniform'])
    \ei
\item Normalizer(norm=a) = randchoice([`l1', `l2',`max'])
  
\item Binarizer(threshold=a) =  randuniform(0,100)
   
    \item SMOTE(a=n\_neighbors, b=n\_synthetics,  c=Minkowski\_exponent)
    \bi
    \item a,b = randit(1,20),randchoice(50,100,200,400)
    \item c = randuniform(0.1,5)
    \ei
\ei

 \\\hline
{\bf Pre-Processors for Text mining:}  
 
\bi
\item CountVectorizer(max\_df=a, min\_df=b) = randint(100, 1000), randint(1, 10)
\item TfidfVectorizer(max\_df=a, min\_df=b, norm=c)
    \bi
    \item a, b,c = randint(100, 1000), randint(1, 10), randchoice([`l1', `l2', None])
    \ei
\item HashingVectorizer(n\_features=a, norm=b)
    \bi
    \item a = randchoice([1000, 2000, 4000, 6000, 8000, 10000])
    \item b = randchoice([`l1', `l2', None])
    \ei
\item LatentDirichletAllocation(n\_components=a, doc\_topic\_prior=b,\newline topic\_word\_prior=c,
                                   learning\_decay=d,
                                   learning\_offset=e,batch\_size=f)
    \bi
    \item a, b, c = randint(10, 50), randuniform(0, 1),  randuniform(0, 1)
    \item d, e  = randuniform(0.51, 1.0), randuniform(1, 50), 
    \item f = randchoice([150,180,210,250,300])
    \ei
\ei 


 \\\hline
 \end{tabular}

\end{table}
